Emergent Flows, Irreversibility and Unsteady Effects in Asymmetric and Looped Geometries

Fluid transport networks are important in many natural settings and engineering applications, from animal cardiovascular and respiratory systems to plant vasculature to plumbing networks and chemical plants. Understanding how network topology, connectivity, internal boundaries and other geometrical aspects affect the global flow state is a challenging problem that depends on complex fluid properties characterized by different length and time scales. The study of flow in micro-scale networks focuses on low Reynolds numbers where small volumes of fluids move at slow speeds. The flow physics at these scales is governed by the Stokes equation, which is linear. This linearity property allows for relatively simple theoretical and computational solutions that greatly aid in the understanding, modeling and designing of micro-scale networks. At larger scales and faster flow rates, macrofluidic networks are also important but the flow physics is quite different. The underlying Navier-Stokes equation is nonlinear, theoretical results are few, simulations are challenging, and the mapping between geometry and desired flow objectives are all much more complex. The phenomenology for such high-Reynolds-number or inertially-dominated flows is well documented and well-studied: Flows are retarded in thin boundary layers near solid surfaces; such flows are sensitive to geometry and tend to separate from surfaces; and vortices, wakes, jets and unsteadiness abound. The counter-intuitive nature of inertial flows is exemplified by the breakdown of reversibility. This dissertation explores two general ways of how rectified flows emerge in macrofluidic networks as a consequence of irreversibility and unsteady effects: When branches or channels of a network have asymmetric internal geometry and the second when a network contains loops.

==> chapters/1-intro.tex <==

From animal cardiovascular and respiratory systems to plant vasculature to plumbing networks and chemical plant, controlling flows is important in many natural settings and engineering applications \cite{nielsen1964animal,conway1971guide,lal1975hydraulic,waite2007applied,fung2013biomechanics}.  Understanding how network topology, connectivity, internal boundary and other geometrical aspects determine the global flow state is a challenging problem that depends crucially on the fluid dynamical regime, which is characterized by dimensionless quantities involving length- and time-scales and fluid material properties \cite{tritton2012physical}. The study of flow  in micro-scale networks including  microvascular network of small animals, plant vasculature \cite{jensen2016sap} and artificial microfluidics \cite{whitesides2006origins} focuses on low Reynolds numbers in which small volumes are conveyed at slow speeds. The flow physics at these scales is dominated by pressures overcoming viscous impedance, and the governing Stokes equation is linear \cite{squires2005microfluidics}. This linearity property enables theoretical and computational solutions that greatly aid in the understanding, modeling and design of micro-scale networks. 


At larger scales and faster flow rates,  macrofluidic networks such as in cardiovascular and respiratory systems of larger animals and numerous engineering applications are also important but the flow physics quite different. The underlying Navier-Stokes equation is nonlinear, theoretical results are few, simulations are challenging, and the mapping between geometry and desired flow objectives all the more complex \cite{tritton2012physical}. The gross phenomenology for such high-Reynolds-number or inertially-dominated flows is well documented and well studied: Flow is retarded in thin boundary layers near solid surfaces; such flows are sensitive to geometry and tend to separate from the surface; and vortices, wakes, jets and unsteadiness abound \cite{schlichting2016boundary}. The counter-intuitive nature of inertial flows is exemplified by the breakdown of reversibility: Running a given system in reverse, say by inverting pressures, does not necessarily cause the fluid to move in reverse but can instead trigger altogether different flow patterns \cite{tritton2012physical}. The controlling of flow in macrofluidic networks must rely on the physics of inertial flow, and the most basic operation is controlling the flow direction or rectification. 


This dissertation explores two strategies that the physics of inertial flows are exploited in combination with complex geometry to achieve circulation or pumping effect. The first relies on complex internal geometry of fluid conduits that make up the \textit{macrofluidic} network and the second, the connectivity of network itself. 


==> chapters/5old.tex <==
\section{Introduction}
A simple sketch model consisting of a single loop and two bifurcation was first suggested by Hazelhoff. However in his model he stresses the important of the guiding dam located at one bifurcation, as well as the curvature of the bronchi. He also thought that the front and back air sac play different roles. 

butler1988-Dotterweich (1936) and Hazelhoff both build glass models to demonstrate that aerodynamic forces were capable of rectification seen in the lung. However they incorporated features (?) not strictely based on avian lung. Kueth has fixed lung model (with air sacs) and was able to generate rectified flow. 

In previous research, inspiratory and expiratory valving are studied separately. 

Our model consists of minimal ingredients for flow rectification: loop topology and mirror geometry, and these are generalizable to more complex network.



==> chapters/piv.tex <==

\subsection*{Reducing distortion}
The index of refraction of the thin tube is slightly different from that of water. Because the tube is thin, the distortion is expected to be minimal. Nevertheless, it's was checked carefully. A ruler was placed inside the tube, and the tube and the water jacket are both filled with water. The the rule with dense tickmarks was photograph. Image processing in MATLAB produces increments of tickmarks in pixels. A linear increments indicates minimal distortion.

\subsection*{Selecting neutrally buoyant microparticles}

\subsection*{Measuring flow rates of steady flow}
The PIV method is compared against a known flow rate in a the tube. 


\subsection*{Measuring flow rates of pulsatile flow}

\subsection*{Parallel processing on a computer cluster}
Terabytes worth of high speed video clips consists of thousands of high resolution frames each, and the processing of each frame is time consuming. A customized parallelized program was developed on MATLAB to process all videos on a computer clusters and compile the result.  

==> defs.tex <==
% ----------------------------------------
% Packages
% ----------------------------------------

% 
% Place here your \usepackage's. Some recommended packages are already included.
%

% Graphics:
%\usepackage[final]{graphicx}
\usepackage{graphicx} % use this line instead of the above to suppress graphics in draft copies
%\usepackage{graphpap} % \defines the \graphpaper command

% Uncomment this to indent first line of each section:
 \usepackage{indentfirst}

% Good AMS stuff:
\usepackage{amsthm} % facilities for theorem-like environments
%\usepackage[tbtags]{amsmath} % a lot of good stuff!

% Fonts and symbols:
\usepackage{amsfonts}
\usepackage{amssymb}

% Set the fonts
\RequirePackage[T1]{fontenc}
\ifxetex
  \RequirePackage[tt=false]{libertine}
\else
  \RequirePackage[tt=false, type1=true]{libertine}
\fi
\RequirePackage[varqu]{zi4}
\RequirePackage[libertine]{newtxmath}


% For typesetting inference rules
\usepackage{mathpartir}
% \usepackage{pftools}  % A local package
\newcommand{\bmmax}{2}
\usepackage{bm}

% Formatting tools:
%\usepackage{relsize} % relative font size selection, provides commands \textsmalle, \textlarger
%\usepackage{xspace} % gentle spacing in macros, such as \newcommand{\acims}{\textsc{acim}s\xspace}

% Page formatting utility:
%\usepackage{geometry}

\usepackage{booktabs}   %% For formal tables:
                        %% http://ctan.org/pkg/booktabs
\usepackage[labelformat=simple]{subcaption} %% For complex figures with subfigures/subcaptions
                        %% http://ctan.org/pkg/subcaption
% Options to subcaption are to label and refer to subfigures as Fig 1(a) etc.
\renewcommand\thesubfigure{(\alph{subfigure})}

\usepackage[T1]{fontenc} % needed for scaling fancy fonts (?)
\usepackage[utf8]{inputenc} % not sure this is needed

\usepackage{amssymb}
%\usepackage[table]{xcolor}

% For code
\usepackage[final]{listings}
\lstset{mathescape=true}

% For code highlighting
% \usepackage{bold-extra}

% Tikz
\usepackage{tikz}
\usetikzlibrary{matrix,arrows,positioning,calc,fit,backgrounds}

% To control enum item labelling/numbering
\usepackage[shortlabels, inline]{enumitem}
% To give custom item labels and reference them
\makeatletter
\newcommand{\myitem}[1][]{
  \protected@edef\@currentlabel{#1}%
\item[#1]
}
\makeatother

% To stop aligned env swallowing up []s
\usepackage{mathtools}

% To use ifstrempty
\usepackage{etoolbox}

% For math mode tables
\usepackage{array}
% A text column in array
\newcolumntype{L}{>$l<$}

% For \llbracket and \rrbracket
\usepackage{stmaryrd}

% For dashed boxes
\usepackage{dashbox}

% For big separating conjunction
\usepackage{scalerel}

% For mathpar environment
\usepackage{mathpartir}

\usepackage{xspace}
\usepackage{multirow}

% To stop citations overflowing lines
\usepackage{breakcites}

% For citet command
% \usepackage{natbib}
% \setcitestyle{%
%     authoryear,%
%     open={[},close={]},citesep={;},%
%     aysep={},yysep={,},%
%     notesep={, }}
% \let\cite\citep
%\usepackage[square,sort,comma,numbers]{natbib}

%%
%% Place here your \newtheorem's:
%%

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[chapter]
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}
\theoremstyle{plain}


% ----------------------------------------
% Generic definitions
% ----------------------------------------
% Required packages: listings, tikz

% A footnote without a marker
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\renewcommand{\le}{\leqslant}
\renewcommand{\ge}{\geqslant}
% \renewcommand{\emptyset}{\ensuremath{\varnothing}}
% \newcommand{\ds}{\displaystyle}

% Math stuff
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\closure}[1]{\ensuremath{\overline{#1}}}
%\newcommand{\acim}{\textsc{acim}\xspace}
%\newcommand{\acims}{\textsc{acim}s\xspace}

\newcommand{\Land}{\bigwedge}
\newcommand{\Lor}{\bigvee}
\newcommand{\es}{\emptyset}
\newcommand{\incl}{\subseteq}
\newcommand{\impl}{\Rightarrow}
\renewcommand{\iff}{\Leftrightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\sat}{\vDash}
\newcommand{\notsat}{\nvDash}
\newcommand{\proves}{\vdash}
\newcommand{\provesIff}{\mathrel{\dashv\vdash}}
\newcommand{\boolTrue}{\top}
\newcommand{\boolFalse}{\bot}

\newcommand{\dom}{\operatorname{\mathsf{dom}}}
\newcommand{\range}{\operatorname{\mathsf{rng}}}
\newcommand{\restrict}[2]{{#1}|_{#2}}
\newcommand{\pto}{\rightharpoonup}

\newcommand{\defeq}{\coloneqq}
\newcommand{\defiff}{\vcentcolon\iff}

\newcommand{\pipe}{\triangleright}

%% Caligraphic
\newcommand{\Aa}{{\mathcal{A}}}
\newcommand{\Bb}{{\mathcal{B}}}
\newcommand{\Cc}{{\mathcal{C}}}
\newcommand{\Dd}{{\mathcal{D}}}
\newcommand{\Ee}{{\mathcal{E}}}
\newcommand{\Ff}{{\mathcal{F}}}
\newcommand{\Gg}{{\mathcal{G}}}
\newcommand{\Hh}{{\mathcal{H}}}
\newcommand{\Ii}{{\mathcal{I}}}
\newcommand{\Jj}{{\mathcal{J}}}
\newcommand{\Kk}{{\mathcal{K}}}
\newcommand{\Ll}{{\mathcal{L}}}
\newcommand{\Mm}{{\mathcal{M}}}
\newcommand{\Nn}{{\mathcal{N}}}
\newcommand{\Oo}{{\mathcal{O}}}
\newcommand{\Pp}{{\mathcal{P}}}
\newcommand{\Qq}{{\mathcal{Q}}}
\newcommand{\Rr}{{\mathcal{R}}}
\newcommand{\Ss}{{\mathcal{S}}}
\newcommand{\Tt}{{\mathcal{T}}}
\newcommand{\Uu}{{\mathcal{U}}}
\newcommand{\Vv}{{\mathcal{V}}}
\newcommand{\Ww}{{\mathcal{W}}}
\newcommand{\Yy}{{\mathcal{Y}}}
\newcommand{\Zz}{{\mathcal{Z}}}

% Wrappers: Parens, brackets, etc
% \newcommand{\op}[1]{\operatorname{#1}}
\newcommand{\paren} [1] {\ensuremath{ \left( {#1} \right) }}
\newcommand{\bigparen} [1] {\ensuremath{ \Big( {#1} \Big) }}
% \newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\tuple}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\abs}[1]{\ensuremath{\lvert #1 \rvert}}
% \newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\setcomp}[2]{\ensuremath{\left\{#1\;\middle|\;#2\right\}}}

% References
\newcommand{\refCh}[1]{Chapter~\ref{#1}}
\newcommand{\refSc}[1]{Section~\ref{#1}}
% \newcommand{\refSc}[1]{\S\ref{#1}}
\newcommand{\refFig}[1]{Figure~\ref{#1}}
\newcommand{\refDef}[1]{Definition~\ref{#1}}
\newcommand{\refLem}[1]{Lemma~\ref{#1}}
\newcommand{\refThm}[1]{Theorem~\ref{#1}}
\newcommand{\refAlg}[1]{Algorithm~\ref{#1}}
\newcommand{\refEx}[1]{Example~\ref{#1}}
\newcommand{\refCor}[1]{Corollary~\ref{#1}}
\newcommand{\refTab}[1]{Table~\ref{#1}}
\newcommand{\refEq}[1]{\ensuremath{(\ref{#1})}}
\newcommand{\refRule}[1]{(\ref{#1})}
\newcommand{\refApp}[1]{Appendix~\ref{#1}}

\newcommand{\tool}[1]{\textsf{#1}}
\newcommand{\code}[1]{\textnormal{\small\texttt{#1}}}
% \newcommand{\code}[1]{\text{\lstinline{#1}}}

% TODO have macros for \forall and \exists

\newcommand{\tick}{\ensuremath{\checkmark}}
\newcommand{\cross}{\text{\sffamily X}}


% ----------------------------------------
% Paper specific macros & commands
% ----------------------------------------


% Put your definitions here


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "thesis"
%%% End:

